Non-monotone Submodular Maximization with Nearly Optimal Adaptivity and Query Complexity

Submodular maximization is a general optimization problem with a wide range of applications in machine learning (e.g., active learning, clustering, and feature selection). In large-scale optimization, the parallel running time of an algorithm is governed by its adaptivity, which measures the number of sequential rounds needed if the algorithm can execute polynomially-many independent oracle queries in parallel. While low adaptivity is ideal, it is not sufficient for an algorithm to be efficient in practice -- there are many applications of distributed submodular optimization where the number of function evaluations becomes prohibitively expensive. Motivated by these applications, we study the adaptivity and query complexity of submodular maximization. In this paper, we give the first constant-factor approximation algorithm for maximizing a non-monotone submodular function subject to a cardinality constraint $k$ that runs in $O(\log(n))$ adaptive rounds and makes $O(n \log(k))$ oracle queries in expectation. In our empirical study, we use three real-world applications to compare our algorithm with several benchmarks for non-monotone submodular maximization. The results demonstrate that our algorithm finds competitive solutions using significantly fewer rounds and queries.

==> maximization.tex <==
\section{\Wrapper Algorithm}
\label{sec:maximization}

In this section we show how the \AdaptiveSampling algorithm fits into a greedy framework
for maximizing monotone submodular functions with a cardinality constraint.
We start by presenting the \Wrapper algorithm, and then we prove its
guarantees in \Cref{sec:wrapper_analysis}.
The algorithm \Wrapper works as follows.
Given an initial threshold~$\tau$, \Wrapper constructs a solution
repeatedly running \AdaptiveSampling 
at decreasing thresholds $(1-\varepsilon)^j \tau$ conditioned on the
current partial solution.
It is greedy in the sense that every time \AdaptiveSampling is called,
the expected average contribution of the elements in the returned set
is at least $(1-\varepsilon)\tau$ and
the marginal gain of all remaining elements
is less than the current threshold.
These properties allow us to prove an approximation guarantee with respect to
the initial choice of threshold $\tau$.

To relate such an approximation to $\OPT$, we let
$\Delta^* = \max\{f(x) : x \in N\}$ be an upper bound for all marginal
contributions by submodularity and
observe that $\Delta^* \le \OPT \le k\Delta^*$.
The threshold that \Wrapper searches for is $\tau^* = \OPT/k$, so
it suffices to run the greedy thresholding algorithm for $O(\log(k)/\varepsilon)$
initial thresholds $(1+\varepsilon)^i \Delta^*/k$ in parallel
and return the solution with maximum value.
Since the algorithm will try some threshold $\tau$
close enough to $\tau^*$, specifically $\tau \le \tau^* \le (1+\varepsilon)\tau$,
the approximation to $\OPT$ follows.
Note that by trying thresholds all in parallel, the adaptivity complexity
of the algorithm does not increase.
In \Cref{sec:linear-queries} we present efficient preprocessing methods that
reducing the ratio of the interval containing $\OPT$.

\begin{algorithm}[H]
  \caption{\Wrapper}
  \label{alg:wrapper}
  \vspace{0.1cm}
  \textbf{Input:} evaluation oracle for $f : 2^N \rightarrow \R$, constraint $k$, error $\varepsilon$, failure probability $\delta$
  \begin{algorithmic}[1]
%    \State \todo{Set smaller error: $\hat{\varepsilon} \leftarrow \varepsilon/2$? Propagate change.}
    \State Set upper bounds $\Delta^* \leftarrow \max\{f(x) : x \in N\}$,
    $r \leftarrow \ceil{2\log(k)/\varepsilon}$,
    $m \leftarrow \ceil{\log(4)/\varepsilon}$
    \State Set smaller failure probability $\hat{\delta} \leftarrow \delta/(r(m+1))$
    \State Initialize $R \leftarrow \emptyset$
    \For{$i=0$ to $r$ in parallel}
      \State Set $\tau \leftarrow (1+\varepsilon)^i \Delta^*/k$
      \State Initialize $S \leftarrow \emptyset$
      \For{$j=0$ to $m$} \Comment{Until $(1-\varepsilon)^j\tau < \tau/4$}
        \State Set $T \leftarrow \AdaptiveSampling(N, f_S, k - |S|, (1-\varepsilon)^j \tau, \varepsilon, \hat{\delta})$
        \State Update $S \leftarrow S \cup T$
        \If{$|S|=k$}
          \State \textbf{break}
        \EndIf
      \EndFor
    \If{$f(S) > f(R)$}
      \State Update $R \leftarrow S$
    \EndIf
    \EndFor
    \State \textbf{return} $R$
  \end{algorithmic}
\end{algorithm} 

\begin{restatable}[]{theorem}{approx}\label{thm:approx_factor}
For any monotone, nonnegative submodular function $f$,
\Wrapper outputs a set $S \subseteq N$ with $|S| \le k$ in
$O(\log(n/\delta)/\varepsilon^{2})$ adaptive rounds such that
with probability at least $1 - \delta$
the algorithm makes $O(n \log(k)/\varepsilon^3)$
oracle queries in expectation and $\E[f(S)] \ge (1 - 1/e - \varepsilon)\OPT$.
\end{restatable}

\subsection{Analysis of the \Wrapper Algorithm}
\label{sec:wrapper_analysis}

To analyze the expected approximation factor of \Wrapper, we first assume
that all calls to \AdaptiveSampling give correct outputs by our choice of
$\hat{\delta}$ and a union bound.
The analysis that follows is for one execution of the block in the
for loop of \Wrapper (Line 5 to Line 13)
and assumes the initial value of $\tau$ is
sufficiently close to $\tau^* = \OPT/k$, satisfying
the inequality $\tau \le \tau^* \le (1+\varepsilon)\tau$.
Furthermore, we assume that $m = \infty$ and that
the final output set is of size~$k$.
We refer to this modified block of \Wrapper as the algorithm.

For a fixed input, as the algorithm runs it produces nonempty sets
$T_1,T_2,\dots,T_m$, inducing a probability distribution over
sequences of subsets.
Denote their respective sizes by $t_1,t_2,\dots,t_m$ and the input values
$(1-\varepsilon)^j \tau$
for which they were returned by $\tau_1, \tau_2,\dots,\tau_m$.
We view the algorithm
as a random process that adds elements to the output set $S$ one at a time
instead of set by set. Specifically, for each new $T_i$ the algorithm adds each $x \in
T_i$ to $S$ in lexicographic order, producing a sequence of subsets
$S_0 \subseteq S_1 \subseteq \dots \subseteq S_k$ with $S_0 = \emptyset$.
Note that there is no randomness
in adding the elements of $T_i$ once $T_i$ is drawn.

Instead of analyzing the expected value of the partial solution $\E[f(S_i)]$ at
each step, we consider an averaged version of this random process that is
easier to analyze and whose final expected value is equal to $\E[f(S_k)]$.
In particular, when the process draws a set $T_\ell$,
each element $x \in T_\ell$ contributes the same amount
$\Delta(T_\ell, T_1 \cup \dots \cup T_{\ell-1})/|T_{\ell}|$ to the value of the
output set.
Formally, we define the averaged version of the random process as
\[
  \hat{f}(S_i) \DEF
  f(T_1 \cup \dots \cup T_{\ell-1}) + 
  \frac{i - (t_1 + \dots + t_{\ell-1})}{t_\ell}
  \cdot
  \Delta(T_\ell, T_1\cup \dots \cup T_{\ell-1}),
\]
where we use the overloaded notation
$S_i = (i, T_1, T_2, \dots, T_\ell)$ to record
the history of the process up to adding the $i$-th element.
This means that
$t_1 + t_2 + \dots + t_{\ell - 1} < i$ and
$t_1 + t_2 + \dots + t_{\ell} \ge i$.
Note that for a given history $T_1,T_2,\dots,T_m$ of subsets, both processes
agree after adding a complete subset.
Analogously, we define the marginal of the $i$-th element $X_i$ of this
process to be
\[
  \hat\Delta(X_i, S_{i-1}) \DEF
  \frac{\Delta(T_\ell, T_1\cup \dots \cup T_{\ell-1})}{t_\ell}.
\]
Since the original algorithm induces a probability distribution over sequences of
returned subsets, this defines a distribution over the
values of $\hat{f}(S_i)$ and $\hat{\Delta}(X_i, S_{i-1})$ for all indices $i \in [k]$.

Lastly, it will be useful to define the distribution $\mathcal{H}$ over all
possible (random bit) histories $(T_1,T_2,\dots,T_m)$
at the termination of the algorithm, and also the distributions
$\mathcal{H}_i$, for all $i \in [k]$, over the
possible histories \emph{immediately} before adding the $i$-th
element. This means that for each $h = (T_1,T_2,\dots,T_{\ell-1}) \in
\text{supp}(\mathcal{H}_i)$ we have
$t_1 + t_2 + \dots + t_{\ell-1} < i$ and
there exists a set~$T_\ell$ that can be drawn such that
$t_1 + t_2 + \dots + t_{\ell} \ge i$.
Let $H_i(h)$ be the event over $\mathcal{H}_i$ such that the history is $h =
(T_1,T_2,\dots,T_{\ell-1})$ and the next returned subset $T_\ell$ adds the
$i$-th element.
We condition our statements on $H_i(h)$, as this captures
the state of the algorithm just before adding the $i$-th element.
To provide intuition for \Cref{lem:expectation_approx},
it is worth noting that $\mathcal{H}$ is a refinement of
$\mathcal{H}_i$ conditioned on $H_i(h)$. This can be seen
by recursively joining leaves in the probability tree of $\mathcal{H}$
until the $i$-th element is reached. The
result is the probability tree of $\mathcal{H}_i$
conditioned on $H_i(h)$.
In the statements that follow, the probabilities and expectations
conditioned on $H_i(h)$ are over the distribution $\mathcal{H}_i$ and
all other expressions are over the distribution $\mathcal{H}$ of final
outcomes.

\begin{lemma} 
\label{lem:conditional_iterative_property}
%For all $i \in [k]$, let $H_i$  be the event that (random bit) history
%is $h = (T_1,\dots,T_{\ell-1})$ and the next returned subset $T_\ell$ adds the
%$i$-element (i.e., $t_1 + \dots + t_{\ell-1} < i$ and $t_1 + \dots + t_\ell \ge i$).
%For $\tau \le \tau^* \le (1+\varepsilon)\tau$, we have
For all $i \in [k]$, events $H_i(h)$ and thresholds $\tau$ such that
$\tau \le \tau^* \le (1+\varepsilon)\tau$, we have
\begin{align*}
  \ExpCond{}{\hat{\Delta}\parens*{X_i, S_{i-1}}}{H_i(h)} \ge
  \frac{\parens*{1-\varepsilon}^2}{k}\cdot\ExpCond{}{\OPT - \hat{f}(S_{i-1})}{H_i(h)}.
\end{align*}
\end{lemma}

\begin{proof}
%Assume that the initial approximation $\tau$ to $\tau^* = \OPT/k$ satisfies
%$\tau^* \le \tau \le (1+\varepsilon)\tau^*$.
First we prove the claim for $i = 1$, and then we proceed by case analysis.
If $i=1$ there is no history, so it suffices to show that
  $E[\hat{f}(S_1)] \ge (1-\varepsilon)^2\OPT/k$.
The first element belongs to the subset $T_1$ returned by
\AdaptiveSampling, so by
Property 2 of \Cref{lem:adaptive_sampling},
it follows that
\begin{align*}
  \Exp{}{\hat{f}\parens*{S_1}}
  &=
  \Exp{}{\frac{f\parens*{T_1}}{\abs*{T_1}}}
  \ge \parens*{1-\varepsilon} \tau
  \ge \parens*{\frac{1-\varepsilon}{1+\varepsilon}} \cdot \frac{\OPT}{k}
  \ge \parens*{1-\varepsilon}^2 \cdot \frac{\OPT}{k}.
\end{align*}

Assuming now that $i > 1$,
let $i^* = t_1 + \dots + t_{\ell - 1} + 1$ be the size of the partial solution
after adding the first element in $T_\ell$.
We consider the cases $i=i^*$ and $i > i^*$ separately.
If $i = i^*$, observe that for monotone submodular functions we have
\begin{align*}
  f\parens*{S^*} &\le f\parens*{S^* \cup S_{i-1}}\\
  &\le f\parens*{S_{i-1}} + \sum_{x \in S^*} \Delta(x, S_{i-1})\\
  &\le f(S_{i-1}) + k \cdot \frac{\tau_{\ell}}{1-\varepsilon} & \text{(Property 3 of \Cref{lem:adaptive_sampling})}\\
  &\le f(S_{i-1}) + \frac{k}{(1-\varepsilon)^2} \cdot \ExpCond{}{\frac{\Delta\parens*{T_\ell, S_{i-1}}}{\abs*{T_\ell}}}{H_i(h)} & \text{(Property 2 of \Cref{lem:adaptive_sampling})}\\
  &= f(S_{i-1}) + \frac{k}{(1-\varepsilon)^2} \cdot \ExpCond{}{\hat{\Delta}\parens*{X_i, S_{i-1}}}{H_i(h)}.
\end{align*}
In the first annotated inequality,
we have $\tau_{\ell}/(1-\varepsilon)$ 
because \AdaptiveSampling was run with this parameter immediately
before running with the threshold $\tau_{\ell}$, which returned $T_\ell$.
The upper bound for the marginal $\Delta(x, S_{i-1})$ for $x \in
S^*$ is then a consequence of Property 3 of \Cref{lem:adaptive_sampling}.

The history $h=(T_1,T_2\dots,T_{\ell-1})$ is known since we
are conditioning on $H_i(h)$, so it follows that
\[
  f\parens*{S^*} - f\parens*{S_{i-1}}
  =
  \ExpCond{}{\OPT - \hat{f}\parens*{S_{i-1}}}{H_i(h)},
\]
because there is no randomness in the expectation.
Recall that $f(S_{i-1}) = \E[\hat{f}(S_{i-1}) \mid H_i(h)]$ because
the set $S_{i-1} = T_{1} \cup \dots \cup T_{\ell-1}$ is a union of complete sets, and hence
there are no partial, averaged contributions.
Rearranging the previous inequalities gives
\begin{align*}
  \ExpCond{}{\hat{\Delta}\parens*{X_i, S_{i-1}}}{H_i(h)}
  \ge \frac{\parens*{1-\varepsilon}^2}{k}\cdot
      \ExpCond{}{\OPT - \hat{f}\parens*{S_{i-1}}}{H_i(h)},
\end{align*}
as desired.

Now we consider the case when $i > i^*$.
Because we condition on the history
$h=(T_1,T_2,\dots,T_{\ell-1})$
immediately before drawing a set $T_\ell$
that necessarily contains the $i$-element,
the averaging property of~$\hat{f}$ and
the analysis for the previous case give us
\begin{align*}
  \ExpCond{}{\hat{\Delta}\parens*{X_i, S_{i-1}}}{H_i(h)}
  &= \ExpCond{}{ \hat{\Delta}\parens*{X_{i^*}, S_{i^* - 1}} }{H_i(h)}\\
  &\ge \frac{\parens*{1-\varepsilon}^2}{k}\cdot
      \ExpCond{}{\OPT - \hat{f}\parens*{S_{i^* - 1}}}{H_i(h)}\\
  &\ge \frac{\parens*{1-\varepsilon}^2}{k}\cdot
      \ExpCond{}{\OPT - \hat{f}\parens*{S_{i-1}}}{H_i(h)}.
\end{align*}
The final inequality makes use of 
$\E[\hat{f}(S_{i-1}) \mid H_i(h)] \ge \E[\hat{f}(S_{i^* - 1}) \mid H_i(h)]$,
which is a consequence of monotonicity and
the averaging property of $\hat{f}$.
This completes the proof for all $i \in [k]$.
\end{proof}

%\begin{lemma}
%\label{lem:prob_tree_flow}
%If for all $i \in [k]$, events $H_i(h)$ and any constant $c > 0$, we have
%\[
%  \ExpCond{}{\delta_i}{H_i(h)}
%  \le c\cdot
%  \ExpCond{}{\delta_{i-1}}{H_i(h)},
%\]
%then
%\[
%  \Exp{}{\delta_i}
%  \le c\cdot
%  \Exp{}{\delta_{i-1}}.
%\]
%\end{lemma}
%
%\begin{proof}
%\todo{This missing proof is critical but seems true via probability tree.}
%\end{proof}


\begin{lemma}
\label{lem:expectation_approx}
If for all $i \in [k]$ and events $H_i(h)$ we have
\[
  \ExpCond{}{\hat{\Delta}\parens*{X_i, S_{i-1}}}{H_{i}(h)} \ge
  \frac{(1-\varepsilon)^2}{k}\cdot\ExpCond{}{\OPT - \hat{f}(S_{i-1})}{H_{i}(h)},
\]
then the algorithm returns a set $S_k$ such that
$\Exp{}{f\parens*{S_k}} \ge \parens*{1 - 1/e - \varepsilon} \OPT$.
\end{lemma}

\begin{proof}
Let $\delta_i = \OPT - \hat{f}(S_i)$, and observe that 
%\[
$
  \ExpCond{}{\Delta\parens*{X_i,S_{i-1}}}{H_i(h)}
  = 
  \ExpCond{}{\delta_{i-1}}{H_i(h)} - \ExpCond{}{\delta_{i}}{H_i(h)}
$
%\]
by the linearity of expectation.
It follows from the assumption that
\[
  \ExpCond{}{\delta_{i}}{H_i(h)} \le \parens*{1 - \frac{(1-\varepsilon)^2}{k}}
  \cdot \ExpCond{}{\delta_{i-1}}{H_i(h)}.
\]
Since $\mathcal{H}_i$ conditioned on the event $H_i(h)$
is a partition of the final outcome distribution $\mathcal{H}$, 
it follows from the law of total probability that
\begin{align*}
  \Exp{}{\delta_{i}} &= \sum_{h \in \text{supp}\parens*{\mathcal{H}_i}}
    \ExpCond{}{\delta_{i}}{H_i(h)} \cdot \Prob{}{H_i(h)}\\
    &\le \parens*{1 - \frac{(1-\varepsilon)^2}{k}} \sum_{h \in \text{supp}\parens*{\mathcal{H}_i}}
      \ExpCond{}{\delta_{i-1}}{H_i(h)} \cdot \Prob{}{H_i(h)}\\
    &\le \parens*{1 - \frac{(1-\varepsilon)^2}{k}} \cdot \Exp{}{\delta_{i-1}}.
\end{align*}
Iterating this inequality over the sequence of expectations $\E[\delta_i]$ and
the using the fact $1-x \le e^{-x}$,
\begin{align*}
  \Exp{}{\delta_k} &\le \parens*{1 - \frac{(1-\varepsilon)^2}{k}}^k \cdot \Exp{}{\delta_{0}}
  \le \parens*{\frac{1}{e} + \varepsilon}\cdot\Exp{}{\delta_{0}}.
\end{align*}
We clearly have
$\E[\hat{f}(S_0)] = \E[f(S_0)]$ and
$\E[\hat{f}(S_k)] = \E[f(S_k)]$
by the construction of $\hat{f}$.
Moreover,
since $f$ is nonnegative we have $\delta_0 = \OPT - \hat{f}(S_0) \le \OPT$,
thus
%\begin{align*}
$
  \Exp{}{f\parens*{S_k}} \ge \parens*{1 - 1/e - \varepsilon} \OPT,
$
%\end{align*}
which completes the proof.
\end{proof}

%\approx*

\begin{proof}[Proof of \Cref{thm:approx_factor}]
The cardinality constraint is satisfied by construction, so we start by
proving the adaptivity complexity of \Wrapper.
Lowering bounding $\OPT$ by $\Delta^*$ takes one adaptive round,
and each execution of the block in the parallelized for loop is independent of
all previous iterations. Therefore, it suffices to bound the adaptivity
complexity of the for loop block (Line 5 to Line 13).
Each invocation of \AdaptiveSampling is potentially dependent on the last
since~$S$ can be updated in each round.
Therefore, because there are $m = O(1/\varepsilon)$ iterations in
the block, the total adaptivity complexity is
$O\parens{m \log(n/\delta) / \varepsilon}
= O\parens{\log(n/\delta)/\varepsilon^{2}}$
by \Cref{lem:adaptive_sampling}.

Now we analyze the query complexiy of the algorithm.
Each call to \AdaptiveSampling behaves as intended with
probability at least $1-\hat{\delta}$, so by our choice of $\hat{\delta}$
and a union bound, all calls to \AdaptiveSampling are correct
with probability at least $1-\delta$.
Assume that this is the case from now on.
By \Cref{lem:adaptive_sampling},
the expected query complexity of \AdaptiveSampling is~$O(n/\varepsilon)$.
Therefore, it follows that the expected query complexity of \Wrapper is
$O(n + rm (n/\varepsilon)) = O(n \log(k)/\varepsilon^{3})$.

To prove the approximation guarantee, first observe that
$\Delta^* \le \OPT \le k \Delta^*$ by submodularity.
Therefore, we know that $\Delta^*/k \le \tau^* \le \Delta^*$.
The values of $\tau$ considered are $(1+\varepsilon)^i\Delta^*/k$, so by
our choice for the number of iterations $r = O(\log(n)/\varepsilon)$,
there exists a $\tau$ satisfying
$\tau \le \tau^* \le (1+\varepsilon)\tau$.
Although we do not know this value of $\tau$, we use its existence to
give a guarantee by taking the maximum over all potential solutions.
Therefore, with probability at least $1 - \delta$ we have
\[
  \Exp{}{f(S)} \ge \parens*{1-1/e-\varepsilon}\OPT
\]
by \Cref{lem:conditional_iterative_property} and \Cref{lem:expectation_approx},
assuming that the returned set satisfies $|S|=k$.
If instead $|S| < k$, then all unchosen elements $x \in N \setminus S$
have marginals $\Delta(x, S) \le \tau/4$ by our choice of $m$
and Property~3 of \Cref{lem:adaptive_sampling}.
Thus for any $\tau \le \tau^*$, 
monotonicity and submodularity give
\begin{align*}
  f\parens*{S^*} &\le f(S) + \sum_{x \in S^*} \Delta(x, S)
    \le f(S) + k \tau / 4
    \le f(S) + \OPT / 4,
\end{align*}
which implies 
$f(S) \ge \parens{1 - 1/4} \OPT \ge \parens{1 - 1/e} \OPT$.
This proves the approximation guarantee.
\end{proof}

